RAC: A Relational Agent Contract for Constraint-Governed Engineering Tasks

Engineering agents must produce artifacts that satisfy exact, coupled constraints. Existing solutions often require agents to make semantic decisions and also derive consequences such as precise geometry or timing from those decisions, leading to failures in constraint-governed engineering tasks. In this paper, we introduce RAC, a harness-agnostic contract for the action and feedback layer of engineering agents. It specifies authoritative observations, semantic actions, tool-based realization, independent verification, and repair evidence. The agent decides which relations an artifact should satisfy; specialized tools derive their concrete consequences. On PCB placement, routing, and repair tasks, RAC achieves the highest clean-pass rate for all nine evaluated models, averaging 90.9%, compared with 74.0% for the strongest baseline, requirements-only delegation. In job-shop scheduling, direct relational actions achieve 96.3% quality pass versus 59.6% for code-mediated delivery with access to the same scheduling backend. Our evaluations on 141 embedded-code tasks across four microcontroller identify the action contract as a source of agent capability: preserving semantic control while delegating mechanically derivable outputs improves the reliability of constrained artifacts.

==> sections/04_pcb_contract.tex <==
\section{Coordinate-Free PCB Intent}
\label{sec:pcb}

\subsection{Capability boundary}

We decompose PCB layout into semantic decisions, geometric realization, and verification. The agent owns semantic decisions and revises them in response to verified evidence. The solver owns coordinates, paths, clearances, and legal placement. Verification combines the PCB design-rule checker with intent-specific oracles. This boundary permits the model to inspect exact geometry while preventing metric values from entering the write path.

\subsection{Typed read path}

At each turn, the agent receives part references, courtyard and pin geometry, the netlist, footprint metadata, existing copper segments, layer and via information, unrouted nets, and the current design-rule-check result. Intent checks are shown in a coarse form that identifies which requirements hold, without revealing numeric distance-to-goal. A registered detailed-view ablation additionally provides numeric errors and tolerances. Copper serialization has a fixed per-net budget and reports any elision. Regression tests verify that the base typed view is byte-identical across representation rungs.

\subsection{Relational vocabulary}

The frozen write vocabulary contains thirteen operation families (Table~\ref{tab:vocab}). Objects are addressed by semantic identifiers such as reference designator, pin, net, or named region. No operation accepts a coordinate or a metric distance. The only free integer is a via budget.

\begin{table}[t]
    \centering
    \caption{Coordinate-free PCB intent vocabulary. The imperative and declarative surfaces share these operations and solver semantics.}
    \label{tab:vocab}
    \small
    \begin{tabularx}{\linewidth}{@{}lX@{}}
        \toprule
        Domain & Operations and decisions \\
        \midrule
        Placement & \code{place\_relative}: proximity between a part and an anchor; \code{group}: functional grouping; \code{align}: shared axis; \code{symmetry}: paired placement around an axis; \code{board\_edge}: association with a named side; \code{keepout}: exclusion around an object; \code{zone}: membership in a named board region. \\
        Routing & \code{net\_class}: width and clearance classes; \code{diff\_pair}: coupled nets; \code{route\_matched}: length-matched groups; \code{layer\_pref}: allowed or preferred layers; \code{via\_budget}: maximum vias; \code{avoid}: exclusion from an object or region. \\
        \bottomrule
    \end{tabularx}
\end{table}

Magnitudes use small, ordered classes. Placement distance is \code{tight}, \code{close}, or \code{loose}; length tolerance is \code{1\%}, \code{5\%}, or \code{10\%}; width and clearance use closed categorical sets. Class-to-metric mappings are solver-side configuration. The agent cannot read or alter them. Named regions come from a nine-element set consisting of the center, four half-boards, and four quadrants.

The vocabulary is exposed through two composition semantics. In the \emph{imperative} surface, one operation is submitted per turn and the solver numerically repairs all active constraints from the current board. In the \emph{declarative} surface, a complete bundle is solved jointly. A third, requirements-only surface permits netlist-level requirements followed by review and acceptance, intentionally omitting relations such as a particular axis, side, or region. This upper rung measures the value of semantic control that disappears under complete delegation.

\subsection{Information-flow invariants}

Geometry-free execution is enforced at parse time. Coordinates may occur in observations; numeric geometry in an intent action is rejected; every accepted action is machine-checkable; and no human geometry repair enters an episode. Magnitude classes could become a covert coordinate channel if they were sufficiently fine-grained. We bound that channel with a small fixed vocabulary and hidden metric mappings. A log-level smuggling test flags action sequences that reconstruct a target position more precisely than the class resolution permits.

\subsection{Execution and independent intent oracles}

All intent forms normalize to a shared constraint model. A seeded simulated-annealing placer realizes placement constraints, and routing directives condition either a grid router or Freerouting. Each constraint has a normalized margin: non-positive values are satisfied and positive values measure violation in class units. The execution report includes realized geometry, constraint status, solver work, and a witness when feasible.

Intent is scored independently from execution. A proximity oracle measures realized pin-to-pin or center distance; an alignment oracle measures deviation from the requested axis; a matching oracle computes the spread of realized copper lengths. These oracles use class semantics fixed in the specification and never consume the solver's own satisfaction label. A clean pass requires zero design-rule violations, complete routing, and satisfaction of every task-specific intent oracle.

\subsection{Infeasibility evidence}

When a bundle cannot be realized, the response schema contains four field groups:
\begin{equation}
z = (\textit{status},\ \textit{core},\ \textit{margins},\ \textit{admissible relaxations}).
\end{equation}
The status distinguishes an individually infeasible constraint, a homogeneous over-constraint, and a heterogeneous conflict. The core is an irreducible conflicting subset under the bounded solver procedure. Margins quantify violations in class units. Admissible relaxations advance one step through a class order or delete a classless constraint, and are solver-tested for restored or improved feasibility. Because the placer is heuristic, feasible reports carry concrete witnesses; infeasibility reports are best-effort under a registered restart budget. Frozen feedback tasks are reverified with a larger budget.

Constraint deletion can trivially make a bundle feasible. Repair quality therefore includes \emph{intent retention}: the fraction of the original constraints still active, coupled with a task-specific reference repair. A repair is successful only if it is feasible, geometrically clean, and preserves at least as much intent and per-change quality as that reference.

